Improving Covariance-Regularized Discriminant Analysis for EHR-based Predictive Analytics of Diseases

Linear Discriminant Analysis (LDA) is a well-known technique for feature extraction and dimension reduction. The performance of classical LDA, however, significantly degrades on the High Dimension Low Sample Size (HDLSS) data for the ill-posed inverse problem. Existing approaches for HDLSS data classification typically assume the data in question are with Gaussian distribution and deal the HDLSS classification problem with regularization. However, these assumptions are too strict to hold in many emerging real-life applications, such as enabling personalized predictive analysis using Electronic Health Records (EHRs) data collected from an extremely limited number of patients who have been diagnosed with or without the target disease for prediction. In this paper, we revised the problem of predictive analysis of disease using personal EHR data and LDA classifier. To fill the gap, in this paper, we first studied an analytical model that understands the accuracy of LDA for classifying data with arbitrary distribution. The model gives a theoretical upper bound of LDA error rate that is controlled by two factors: (1) the statistical convergence rate of (inverse) covariance matrix estimators and (2) the divergence of the training/testing datasets to fitted distributions. To this end, we could lower the error rate by balancing the two factors for better classification performance. Hereby, we further proposed a novel LDA classifier De-Sparse that leverages De-sparsified Graphical Lasso to improve the estimation of LDA, which outperforms state-of-the-art LDA approaches developed for HDLSS data. Such advances and effectiveness are further demonstrated by both theoretical analysis and extensive experiments on EHR datasets.

==> nonsparse-glasso.tex <==
\begin{table}
\caption{$\left(|\bar\Sigma_l^{-1}-\hat\Theta|_1-|\bar\Sigma_l^{-1}-\hat T|_1\right)$ with varying $\lambda$ (positive values mean $\hat T$ is closer to $\bar\Sigma_l^{-1}$)}\label{tab:table12}
\begin{center}
\small{\begin{tabular}{r|ccc}\hline
Samples ($\times 2$) & $\lambda=1$	& $\lambda=10$	& $\lambda=100$\\\hline
50	&	47.17	&	7.12		&	0.76 \\
100	&	51.42	&	7.21		&	0.76 \\
150	&	53.41	&	7.25		&	0.76 \\
200	&	55.90	&	7.32		&	0.76 \\\hline
\end{tabular}}
\end{center}
\vspace{-5mm}
\end{table}

==> proof.tex <==
\appendix
\section{Appendix}

\subsection{Proof of Theorem 1.}
\begin{proof}
To prove Theorem 1., we first use Cauchy inequality:
 \begin{equation*}
	\begin{aligned}
& \varepsilon(\hat\Sigma,  \Sigma) \\
 &\leq \Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||}{2} \text{  } \frac{||\hat\Sigma^{-1}(\bar\mu_+-\bar\mu_-)||}{||\hat\Sigma^{-1} (\bar\mu_+-\bar\mu_-)||_\Sigma}\right)\\
&\text{Consider the Cholesky Decomposition $\Sigma=M^TM$,} \\
&\text{where $M$ is a full rank square matrix.} \\
&	 \leq \Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||}{2} \text{  } \frac{||M^{-1}||_F  ||M\hat\Sigma^{-1}(\bar\mu_+-\bar\mu_-)||}{||M\hat\Sigma^{-1}(\bar\mu_+-\bar\mu_-)||}\right)\\
&=\Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||}{2}||M^{-1}||_F  \right)\\
&\leq \Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||}{2}\sqrt{||M^{-1}(M^{-1})^T||_F}  \right) \\
&\text{Consider the Cholesky Decomposition $\Sigma^{-1}$ = $(M^{-1})^T$ $M^{-1}$} \\
&\text{(Because $\Sigma^{-1}$ is positive-definite and symmetric.)}\\
&=\Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||}{2}\sqrt{||\Sigma^{-1}||_F}  \right)\\
 &\leq \Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||}{2}\sqrt{||\hat\Sigma^{-1}||_F+||\Sigma^{-1}-\hat\Sigma^{-1}||_F}  \right) 
	\end{aligned} 	
  \end{equation*}
\end{proof}

\subsection{Proof of Theorem 2.}
\begin{proof}
Given any LDA classifier $f_{\hat\Sigma}(x):X\to\{+1,-1\}$, we define the misclassification function $\mathbf{1}[l\neq f_{\hat\Sigma}(x)]=1$ when $l\neq f_{\hat\Sigma}(x)$ and  $\mathbf{1}[l\neq f_{\hat\Sigma}(x)]=0$ when $1=f_{\hat\Sigma}(x)$. Then, the misclassification rate of $f_{\hat\Sigma}(x)$, for any data distribution with density functions $P(x,l)$ and  $l\in\{+1,-1\}$, can be written as:
  \begin{equation*}
	\begin{aligned}
&P[l*f_{\hat\Sigma}(x))<0]\\
&=\sum_{l\in\{+1,-1\}}\int_x\mathbf{1}[l\neq f_{\hat\Sigma}(x)]P(x,l)d_x,
&\text{Consider the density functions $P_{\Sigma^*}(x|l)$ for Gaussian distribution $\mathcal{N}(\bar\mu_l,\Sigma^*)$  and and $l\in\{+1,-1\}$.}\\
&=\sum_{l\in\{+1,-1\}}\int_x\mathbf{1}[l\neq f_{\hat\Sigma}(x)]P(l)*P_{\Sigma^*}(x|l)d_x+\\
&\sum_{l\in\{+1,-1\}}\int_x\mathbf{1}[l\neq f_{\hat\Sigma}(x)]P(l)(P(x|l)-P_{\Sigma^*}(x|l)))d_x\\
&\text{Consider the misclassification rate on Gaussian distribution $\varepsilon(\hat\Sigma,\Sigma^*)$.}\\
&\leq \varepsilon(\hat\Sigma,\Sigma)+ \sum_{l\in\{+1,-1\}}\pi_l\int_x |P(x|l)-P_{\Sigma^*}(x|l))|d_x\\
&\text{Consider Pinsker's inequality.}\\
&\leq\varepsilon(\hat\Sigma,\Sigma^*)+ \sum_{_{l\in\{-1,+1\}}}\pi_{_l}\sqrt{\frac{D_{_\mathrm{KL}}(P_{_l}\|\mathcal{N}_{(\Sigma^*,\bar\mu_l)})}{2}}
	\end{aligned} 	
  \end{equation*}   
\end{proof}

\subsection{Proof of $\hat T$ Convergence Rate}
\begin{proof}
According to~\cite{jankova2015confidence}, suppose $\Sigma$ refers to the true population covariance matrix of a unknown Gaussian distribution and $\hat T$ refers to the de-sparsified Graphical Lasso estimator based on $m$ data samples drawn from the distribution, under specific sparsity assumption:
%
\begin{equation}
d=o(\sqrt{m}/log \ p )
\label{eq:assumptions}
\end{equation}
%
there exists 
%
$$||\hat T-\Sigma^{-1}||_\infty=\mathcal{O}_p\left(\sqrt{log\text{ }p/m}\right),$$
%
where $p$ and $m$ refer to the dimension and sample size, respectively; $d$ refers to the maximal vector support of the population inverse covariance matrix $\Sigma^{-1}$ i.e.,
%
$$d={max}_{1\leq i\leq p}|\{j:\Sigma^{-1}_{i,j}\neq 0\}|;$$ 
%
further $o(\cdot)$ and $\mathcal{O}_p(\cdot)$ are little-o notation and big-O in probability (the notations were defined in~\cite{chernoff1956large}) respectively. 
%
Then, we can further conclude
\begin{equation}
\begin{aligned}
&||\hat T-\Sigma^{-1}||_F=\sqrt{\sum_{1\leq i\leq p}\sum_{1\leq j\leq p}|(\hat T-\Sigma^{-1})_{i,j}|^2} \\
&\sqrt{\left(\sum_{1\leq i\leq p}\sum_{1\leq j\leq p}|(\hat T-\Sigma^{-1})_{i,j}|\right)^2}\\
&\leq p * ||\hat T-\Sigma^{-1}||_\infty\\
& = \mathcal{O}_p\left(\sqrt{p*log\text{ }p/m}\right).
\end{aligned}
\label{eq:conv}
\end{equation}
\end{proof}
%
%\begin{theorem}
%  \begin{equation}
%	\begin{aligned}
%&P[l*f_{\hat\Sigma}(x)<0]\\
%&\leq \Phi\left(-\frac{||\bar\mu_+-\bar\mu_-||_2}{2}\sqrt{||\hat\Sigma^{-1}||_F+||\hat\Sigma^{-1}-\tilde\Sigma^{-1}||_F}\right)\\
%&+ \underset{\Sigma\geq 0}{\mathbf{min}}\left\{\sum_{_{l\in\{-1,+1\}}}\pi_{_l}\sqrt{\frac{D_{_\mathrm{KL}}(P_{_l}\|\mathcal{N}{(\Sigma,\bar\mu_l)})}{2}}\right\}
%	\end{aligned} 	
%  \end{equation}   
%\end{theorem}



==> tab-nplda.tex <==
\begin{table*}
%\vspace{-0.14in}
\caption{Performance Comparison between \TheName\ and LDA Baselines (Testing Sample Size =$1000\times 2$), where ``ACC.'' refers to accuracy and ``F1.'' refers to F1-Score.%\vspace{-5mm}
}
		\label{tab:table11}
\begin{center}
{
\begin{tabular}{*{12}{c}}
\toprule
    & & \multicolumn{8}{c}{Training Set $\times 2$}\\
    \cmidrule(lr){3-12}
    & &
    \multicolumn{2}{c}{50} &
    \multicolumn{2}{c}{100} &
    \multicolumn{2}{c}{150} &
    \multicolumn{2}{c}{200} &
     \multicolumn{2}{c}{250} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}

Algos & Params & \texttt{ACC.} & \texttt{F1.} &
									   	 \texttt{ACC.} & \texttt{F1.} &
                          			 \texttt{ACC.} & \texttt{F1.} &
                           			 \texttt{ACC.} & \texttt{F1.}  &
                           			 \texttt{ACC.} & \texttt{F1.} \\

\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
LDA&&0.548&0.536&0.599&0.594&0.620&0.621&0.630&0.637&0.643&0.643\\

\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
DIAG&&0.564&0.498&0.606&0.576&0.619&0.608&0.616&0.608&0.634&0.636\\


\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
Ye-LDA&&0.627&0.644&0.620&0.657&0.652&0.688&0.620&0.678&0.655&0.698\\

\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
&0.25&0.559&0.462&0.595&0.522&0.610&0.552&0.624&0.625&0.636&0.639\\
Shrink&0.5&0.558&0.459&0.591&0.517&0.606&0.552&0.612&0.565&0.639&0.639\\
&0.75&0.556&0.412&0.589&0.519&0.620&0.615&0.614&0.566&0.625&0.574\\


\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
 &1.0&0.653&0.673&0.680&0.714&\textbf{0.682}&0.718&0.682&0.723&0.682&0.724\\
CRDA &10.0&0.663&0.702&0.670&0.719&0.677&0.722&0.674&0.721&0.669&0.720\\
&100.0&0.663&0.707&0.663&0.717&0.671&0.722&0.670&0.720&0.663&0.718\\


\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
 					 &1.0&0.650&0.659&\textbf{0.681}&0.703&0.679&0.704&\textbf{0.685}&0.716&\textbf{0.688}&0.719\\
{\TheName} &10.0&\textbf{0.665}&0.700&\textbf{0.681}&\textbf{0.725}&0.681&\textbf{0.724}&0.679&\textbf{0.724}&0.680&\textbf{0.726}\\
 					 &100.0&\textbf{0.665}&\textbf{0.708}&0.665&0.718&0.673&0.722&0.672&0.721&0.666&0.719\\



\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
LR&&0.601&0.436&0.607&0.422&0.603&0.440&0.575&0.318&0.619&0.492\\

\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
SVM &&0.627&0.619&0.642&0.646&0.642&0.646&0.653&0.669&0.661&0.670\\


\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
{AdaBoost}&10&0.635&0.565&0.641&0.554&0.615&0.488&0.597&0.414&0.624&0.508\\
&50&0.624&0.521&0.644&0.560&0.614&0.482&0.612&0.465&0.622&0.502\\


\bottomrule

\end{tabular}
}
\end{center}
\label{tab:main-result}
%\vspace{-5mm}
\end{table*}

